Computational complexity and memory usage for multi-frontal direct solvers in structured mesh finite elements

The multi-frontal direct solver is the state-of-the-art algorithm for the direct solution of sparse linear systems. This paper provides computational complexity and memory usage estimates for the application of the multi-frontal direct solver algorithm on linear systems resulting from B-spline-based isogeometric finite elements, where the mesh is a structured grid. Specifically we provide the estimates for systems resulting from $C^{p-1}$ polynomial B-spline spaces and compare them to those obtained using $C^0$ spaces.

==> PaxHeader/Estimates.tex <==
18 gid=1840429327
18 uid=2022889333
20 ctime=1333870833
20 atime=1333871770
24 SCHILY.dev=234881026
22 SCHILY.ino=8034385
18 SCHILY.nlink=1


==> PaxHeader/alg.tex <==
18 gid=1840429327
18 uid=2022889333
20 ctime=1323252505
20 atime=1333871770
24 SCHILY.dev=234881026
22 SCHILY.ino=4037964
18 SCHILY.nlink=1


==> PaxHeader/complexity.tex <==
18 gid=1840429327
18 uid=2022889333
20 ctime=1323252505
20 atime=1333871770
24 SCHILY.dev=234881026
22 SCHILY.ino=4037965
18 SCHILY.nlink=1


==> PaxHeader/conc.tex <==
18 gid=1840429327
18 uid=2022889333
20 ctime=1323252505
20 atime=1333871770
24 SCHILY.dev=234881026
22 SCHILY.ino=4037966
18 SCHILY.nlink=1


==> PaxHeader/intro.tex <==
18 gid=1840429327
18 uid=2022889333
20 ctime=1323252505
20 atime=1333871770
24 SCHILY.dev=234881026
22 SCHILY.ino=4037969
18 SCHILY.nlink=1


==> PaxHeader/results.tex <==
18 gid=1840429327
18 uid=2022889333
20 ctime=1333871713
20 atime=1333871770
24 SCHILY.dev=234881026
22 SCHILY.ino=8035080
18 SCHILY.nlink=1

